Tracing Water Masers at their Smallest Scale with VLBI

The high-mass star-forming region NGC6334I-MM1 underwent an energetic accretion event in January 2015. We report the large-scale ($10 - 100$ AU) and small-scale ($\sim 1$ AU) changes in spatial and velocity structures of 22 GHz water masers as observed with VERA before and during the accretion burst. The masers in the northern bow-shock CM2-W2 brightened, and better traced a bow structure during the burst. In the southern regions, there was both activation and disappearance of associations before and during the burst. We measured the amplitudes, central velocities and FWHMs of about 20 features in each epoch. We found that the linear scale of the brightest feature in CM2-W2 grew from 0.6 AU before the burst to 1.4 AU after the burst, possibly indicating that a larger volume of gas was able to sustain masing action as a consequence of the accretion burst. This feature also had a rapid (0.2 yr) brightness increase by a factor of four, which has been previously reported in long-term single-dish monitoring. We propose that the water maser flare could be explained by an increase of the collisional pump rate due to radiative heating of H$_2$ by increased high energy radiation (UV or X-ray) from the inner protostellar core. We also describe the spot and spectral method of maser proper motion calculations. We argue that for high spectral resolution observations the spectral method is more robust for calculating proper motions than the spot method.

==> Notes.tex <==
Notes to help me in writing the conference proceedings:

Things todo:

    Write:
        Introduction.
        Method.
        Results.
        Discussion.
        Conclusion.

Introduction - 

Method - The KaVA observations, look at JOC21 paper.

Results -   Showing the main results for the KaVA epoch microstructures. 
    1. Identify microstructures with IMProV.
        Ep1
            Do fits, and identify bad fits.         - DONE
            Do bad fits.
            Make final table.
        Ep2
            Do fits, and identify bad fits.         - DONE
            Do bad fits.
            Make final table.
        Ep3
            Do fits, and identify bad fits.        
            Do bad fits.
            Make final table.
    2. Calculate physical quantities for microstructures.
        Gaussian Parameters -  Peak, FWHM, Centre
        Anything else?
        
    3. Make summary table and plot.
    4. Put in proceedings and describe.

Discussion - Describe physics of microstructures. 
    Previous papers.
    Proper motion methods.
    Velocity drift and effect for proper motions.
